Scalable Variational Gaussian Processes for Crowdsourcing: Glitch Detection in LIGO

In the last years, crowdsourcing is transforming the way classification training sets are obtained. Instead of relying on a single expert annotator, crowdsourcing shares the labelling effort among a large number of collaborators. For instance, this is being applied to the data acquired by the laureate Laser Interferometer Gravitational Waves Observatory (LIGO), in order to detect glitches which might hinder the identification of true gravitational-waves. The crowdsourcing scenario poses new challenging difficulties, as it deals with different opinions from a heterogeneous group of annotators with unknown degrees of expertise. Probabilistic methods, such as Gaussian Processes (GP), have proven successful in modeling this setting. However, GPs do not scale well to large data sets, which hampers their broad adoption in real practice (in particular at LIGO). This has led to the recent introduction of deep learning based crowdsourcing methods, which have become the state-of-the-art. However, the accurate uncertainty quantification of GPs has been partially sacrificed. This is an important aspect for astrophysicists in LIGO, since a glitch detection system should provide very accurate probability distributions of its predictions. In this work, we leverage the most popular sparse GP approximation to develop a novel GP based crowdsourcing method that factorizes into mini-batches. This makes it able to cope with previously-prohibitive data sets. The approach, which we refer to as Scalable Variational Gaussian Processes for Crowdsourcing (SVGPCR), brings back GP-based methods to the state-of-the-art, and excels at uncertainty quantification. SVGPCR is shown to outperform deep learning based methods and previous probabilistic approaches when applied to the LIGO data. Moreover, its behavior and main properties are carefully analyzed in a controlled experiment based on the MNIST data set.

==> z_notUsed_infoLIGOdata.tex <==

\subsection{Classifications file}

Annotations by the citizens. The columns are:
\begin{itemize}
    \item \textit{created at}: date of annotation.
    \item \textit{id}: Unique id for each annotation. \textcolor{red}{Check it and remove repeated annotations if there are.}
    \item \textit{links\_project}: Not useful, all the same value 1104.
    \item \textit{links\_subjects}: Identifier of the image in the Zooniverse platform. There is no a one-to-one correspondence with the images. One image may have several links\_subjects associated (but not the reverse). 
    \item \textit{links\_user}: Identifier of the user. \textcolor{red}{There should not be annotator 0 (not logged in).}
    \item \textit{links\_workflow}: The five levels: 1610 (1), 1934 (2), 1935 (3), 2360 (4), 2117 (5).
    \item \textit{metadata\_finished\_at}: Not useful. 
    \item \textit{metadata\_started\_at}: Not useful.
    \item \textit{metadata\_workflow\_version}: Not useful.
    \item \textit{annotations\_value\_choiceINT}: label as an integer.
    \item \textit{uniqueID}: unique id for each image. Corresponds with links\_subjects as described above.
    \item \textit{annotations\_value\_choice}: label as a string.
\end{itemize}


\subsection{Obtaining LIGO data}
The following Python packages must be installed thorugh pip (still not available in conda):
\begin{itemize}
    \item pip install gwpy
    \item pip install SQLAlchemy
    \item pip install psycopg2-binary
\end{itemize}
The following lines of code obtain the features (last layer of the DNN) for the available images (deeplayertable.ipynb, in forta):
\begin{itemize}
    \item from gwpy.table import EventTable
    \item deeplayer\_data = EventTable.fetch('gravityspy','deeplayer',user='mla',passwd='gl1tch35Rb4d!')
    \item deeplayer data is a certain object that can be converted to numpy or pandas.
\end{itemize}

Information about how to get GravitySpy data: https://gravity-spy.github.io/index.html

For instance, training data can be downloaded as in trainingdata.ipynb.

\subsection{The current system}
\noindent A machine learning method (a CNN) is trained with the golden set.
\begin{itemize}
    \item How is this golden set? Who decided its labels? Does it contain all the 22 classes? Also the ``none of the above'' class? \textcolor{blue}{Manually labelled by Scotty and Mark. All classes, including ``none of the above'', which refers to glitches that are not one of the other 20 types (plus ``no glitch'' class).}
    \item Is this golden set labelled by the annotators, or is it only used to train the neural net?
    \textcolor{blue}{It is also labelled by the annotators. In fact, along with the retired images, these are the only instances whose real label is known. These are necessary to estimate the expertise of the different annotators (which, in turn, is used for the promotion system).}
\end{itemize}

The images to be annotated are passed through the trained NN, which yields a prediction (a 22-dimensional vector that adds up to 1). According to this prediction, the image is assigned to a certain level of difficulty. Level 1 has only 2 classes (plus the ``none of the above''), level 2 has 5 (plus the ``none of the above''), level 3 has 10 (plus the ``none of the above''), and levels 4 and 5 have all the 22.

Annotations are provided by annotators, who can promote when performing well.
\begin{itemize}
    \item How is the promotion system? How do you know when an annotator is ``performing well'' if a real label is not available? \textcolor{blue}{It is based on their performance on those instances whose label is known, i.e. the golden set and the retired images. See the overleaf report by Emre and Neda for more details.}
\end{itemize}

When a certain security about the real label of an instance is achieved, the image is retired and moved into the golden set. Then, the machine is re-trained.
\begin{itemize}
    \item How is the retiring process? When is it considered that the real label is known?
    \textcolor{blue}{When the average of the predictions by the machine and the humans is above a threshold. This ``average'' is explained in the report by Emre and Neda and we proposed some improvements.}
    \item After re-training the machine, its predictions change. Therefore, images might be assigned to a different level according to the current state of the machine. Can this happen? In such a case, the same image could be labelled in different levels (which I thought is not possible). 
    \textcolor{blue}{The assignment of levels is based only on the predictions obtained with the original golden set. It is not updated later.}
\end{itemize}

A final question: What is the ultimate goal of this process? To have the dataset labelled with real (as real as possible) labels? Will this dataset be used just to train a final machine learning model which allows for predicting the class of a new previously-unobserved glitch? In such a case, notice that crowdsourcing methods are machine learning methods which do not need real labels to be trained (just the noisy annotations). Therefore, they would allow for circumventing all this sophisticated process of levels, which is designed to obtain ``real annotations'' (which, of course, are not easy to obtain). This is a great benefit of crowdsourcing methods, which can be seen in fact as the next step to Gravity Spy project.

% \subsection{Free parameters}
% Aspects that could be improved/addressed in the current state of the \emph{retirement} system. By Scotty.
% \begin{itemize}
%     \item The level in which an annotation is made could be considered (although this may compensate at the end, because in higher levels we have better annotators but the instances are more difficult).
%     \item How many annotations have been provided could be also considered. We could trust more in retiring instances for which there are a lot of annotations. 
%     \item Are some classes inherently easier? Could this be included somehow?
%     \item Consider the skill of the annotator.
% \end{itemize}


\subsection{Ideas for the DL+CR/CS+LIGO paper}

Random ideas:

\begin{itemize}
\item Previous papers where the network and golden set are described (check the list in GravitySpy github, \url{https://gravity-spy.github.io/index.html}): \url{https://www.sciencedirect.com/science/article/pii/S0020025518301634}

\item Message from Mike Zevin with papers about citizen science and ML: 
\textit{Hi Pablos, 
here are a few of the citizen science+ML papers that I mentioned, all related to Zooniverse projects. 
Fusion of ML and volunteer classifications: \url{http://arxiv.org/abs/1707.05223}, \url{http://arxiv.org/abs/1802.08713}.
Weighting scheme for volunteers: \url{https://arxiv.org/pdf/1205.6769.pdf}, \url{https://arxiv.org/pdf/1504.06148.pdf}
}
\end{itemize}

Ideas in my mobile phone:
\begin{itemize}
    \item Explote crowdsourced and real labels jointly (novelty in the model!!!)
\item Real labels are used to create a level system so that annotators are more reliable.
\item Algorithms: cnn and cr-cnn (could a prior be added for the annotators so that it is not exactly the same as Rodrigues? Add some info specific to our problem? Maybe in a nature paper the most important part is the application and you do not need to develop new theory? See some previous papers)
\item Citizen science in Science journal:
http://science.sciencemag.org/content/361/6398/134
\end{itemize}

General idea of the paper:
\begin{itemize}
    \item Message: through cutting-edge Deep Learning and Citizen Science (crowdsourcing) techniques, any person in the world can take part in a nobel-awarded high-level project such as LIGO.
    \item LIGO is sensitive. Many glitches. Hard to be labelled by an expert. Crowdsourcing. Mathematical model must account for this citizen science setting. We rely on Deep Learning (most reliable) and add crowdsourcing layer. In order to train (and also to motivate) annotators (which should be truthful on average), we use a levels-based system (their current one). We tailor the DL+CR-layer to our problem, learning also from the data annotated by experts (which is used for the levels system). This is what PRM called ``el mixto''. We compare this with a CNN trained on the golden set.
\end{itemize}

Random ideas, doubts, questions:
\begin{itemize}
    \item Same annotator labelling the same image more than once (no matter whether there are contradictions or not) can be naturally integrated in the model. In fact, it would be like adding a new row with the same features.
    \item About the labels: how does the ``none of the above'' class work? I mean, if the user is only shown class 0, 1, and 2, then ``none of the above'' represents 3 through 21. But if is more options are shown, then ``none of the above'' changes its meaning. Moreover, in such a case, it could not be directly used in our model (we should remove its appearances). \textcolor{red}{``None of the above'' coming from levels 1, 2, 3 (where the user is not shown all the possibilities) should be removed.}
    \item We could take classes that users are more confused about. 
    \item We can use full matrices for the annotators given the underlying real labels with \emph{Dirichlet} priors.
    \item Instances or annotators with only one annotations could be removed. I think it should not be done for instances, since they are useful instances in any case. For annotators, I think they could be removed as long as the number of images does not decreases much.
\end{itemize}
